Achievability of CSS codes performance limits over Pauli channels under separate ML decoding with bounded graphical complexity

Capacity-approaching quantum error correction faces a fundamental tension: the required parity-check matrices need to become increasingly dense, while practical decoding and syndrome extraction favor sparse, bounded-degree structures. Reconciling these competing requirements remains an important open problem in quantum code design. We construct Calderbank-Shor-Steane (CSS) code ensembles that approach the CSS rate over memoryless Pauli channels under maximum-likelihood decoding while retaining sparse, bounded-degree graphical representations. The construction separates parity-check density from graphical complexity: although capacity-approaching components may require dense parity-check matrices, they are represented by sparse concatenated factor graphs. We first study a construction combining low-density parity-check (LDPC) and low-density generator-matrix (LDGM) component codes and numerically analyze the average weight distributions of the resulting codes. Motivated by these results, we introduce a second construction based on concatenated LDPC and LDGM codes and generalized irregular repeat-accumulate (GIRA) codes. We derive bounds on the average weight distribution of the resulting sum ensemble and use the Miller-Burshtein framework to prove simultaneous reliability of the two CSS decoding components. Consequently, the proposed ensemble achieves rates arbitrarily close to the CSS hashing bound under separate bit- and phase-error correction, while maintaining bounded graphical complexity, thus providing a foundation for future iterative decoders and indirect syndrome-extraction architectures.

==> intro_old.tex <==

Low-density parity-check (LDPC) codes, introduced by Gallager~\cite{Gallager1962}, are a fundamental class of classical error-correcting codes whose sparse parity-check matrices admit efficient graphical representations and iterative decoding algorithms. Suitably designed LDPC ensembles can approach channel capacity; however, in conventional LDPC constructions, approaching capacity under iterative decoding generally requires increasing node degrees and, consequently, increasing graphical complexity \cite[Ch.~3.15, pp.~109-112]{RichardsonUrbanke2008}. This motivates the study of sparse code ensembles that retain bounded graphical complexity while exhibiting capacity-achieving performance.

An important development in this direction is the use of concatenated sparse codes.
Pfister, Sason, and Urbanke~\cite{Pfister2004IRA} established capacity-achieving constructions based on irregular repeat--accumulate (IRA) codes for the binary erasure channel. 
%IRA codes may be viewed as sparse concatenated constructions consisting of an outer repetition structure followed by an accumulator. 
Subsequently in ~\cite{HsuAnastasopoulos2005} they considered closely related sparse concatenated ensembles and established capacity-achieving behavior under maximum-likelihood (ML) decoding over memoryless binary-input output-symmetric channels while maintaining bounded graphical complexity.
These results demonstrate that capacity-achieving code ensembles can be constructed using sparse graphical representations, even when their corresponding parity-check matrices are dense.


A central tool for studying ML performance is the average weight distribution of a code ensemble. In particular, the bound of Miller and Burshtein~\cite{Miller2001} relates the ensemble-average ML block error probability to its weight spectrum. The relevant analysis separates the small-weight region, where codewords must be sufficiently suppressed, from weights bounded away from the endpoints, where the average spectrum can be compared with that of a random linear code. This approach is especially useful for structured ensembles whose graphical representations remain sparse even when the corresponding parity-check matrices are not sparse.


ML decoding provides a useful theoretical benchmark for establishing the fundamental performance of a code ensemble. In particular, the ML error probability can be related to the average weight distribution, which makes ML decoding especially suitable for the asymptotic analysis considered in this work. However, exact ML decoding of general linear codes is computationally intractable in the worst case~\cite{xu2007complexity}. Therefore, an ML capacity-achieving result alone does not provide a practical decoding algorithm.

The computational difficulty of ML decoding naturally motivates the use of lower-complexity iterative decoding algorithms. In particular, the sparse graphical representation of LDPC-type codes makes belief-propagation (BP) decoding especially attractive, since BP exploits the local structure of the factor graph through iterative message passing rather than performing a global search over the codebook~\cite{SteendamMoeneclaey2002,Kschischang2001}. Although BP is generally suboptimal compared with ML decoding on graphs containing cycles, it provides a practical decoding method whose complexity is closely tied to the sparsity of the underlying graph. Thus, while ML decoding serves as a theoretical benchmark for establishing the fundamental performance of a code construction, retaining a sparse graphical representation provides a foundation for investigating its performance under practical BP decoding. This motivates the study of BP decoding for the proposed constructions as a natural direction for future work.


The success of sparse graphical constructions in classical coding theory naturally raises the question of whether similar ideas can be applied to quantum error correction. Among quantum error-correcting codes, Calderbank--Shor--Steane (CSS) codes provide a direct connection between classical and quantum coding theory \cite{CalderbankShor1996,steane1996simple}.
%The success of sparse graph--based constructions in classical coding theory naturally raises the question of whether similar ideas can be used to protect quantum information. Quantum states are particularly sensitive to interactions with the environment, which may destroy the coherence needed for quantum communication and computation. Quantum error correction addresses this problem by encoding a smaller number of logical qubits into a larger Hilbert space so that the encoded quantum information can be recovered in the presence of noise \cite{CalderbankShor1996,steane1996simple}. 
A CSS code is constructed from two binary linear codes satisfying an appropriate dual-containing condition. This structure allows the quantum error-correction problem to be decomposed into two classical coding problems associated with bit and phase errors. Consequently, properties of the underlying classical codes---such as their rates, weight distributions, sparse graphical representations, and decoding performance---can be exploited directly in the design and analysis of the resulting quantum code \cite{CalderbankShor1996,steane1996simple}. The central challenge is to achieve the classical reliability requirements while preserving both the CSS nesting condition and a sparse graphical representation. 

% We consider transmission over a memoryless Pauli channel, where each qubit is independently affected by one of the Pauli operators $I$, $X$, $Y$, or $Z$ with probabilities $p_I,p_X,p_Y$, and $p_Z$, respectively. The Pauli errors can be separated into bit- and phase-error components: $X$ contributes a bit error, $Z$ contributes a phase error, and $Y$ contributes both. This structure makes CSS codes particularly natural for Pauli channels, since the two underlying classical codes can be used to protect against the bit- and phase-error components separately. The corresponding channel model and achievable-rate conditions are described more precisely in \ref{sec:achievable_ss}.


In this work, we investigate two constructions of CSS codes based on classical sparse-graph code ensembles. Our objective is to develop CSS constructions that satisfy the required nesting condition while preserving
sparse graphical representations and achieving strong asymptotic performance under ML decoding. We first introduce Construction~A as a simple framework and numerically investigate the ML decoding performance of its classical components through their average weight distributions. The numerical results motivate Construction~B, which extends the initial framework to enable an analytical capacity-achievability result.

Our main theoretical contribution is to establish the capacity-achieving performance of Construction~B under ML decoding. The analysis is based on deriving bounds on the asymptotic average weight distribution of a structured classical code ensemble and applying the achievability framework of Miller and Burshtein~\cite{Miller2001}. Combining this analysis with previously established capacity-achieving results for LDPC/GM ensembles~\cite{HsuAnastasopoulos2005}, we show that the two classical decoding problems associated with the CSS construction can be made simultaneously reliable under ML decoding. Consequently, the proposed CSS construction achieves rates arbitrarily close to the CSS hashing bound under separate bit- and phase-error correction, while retaining a sparse graphical representation. Although this result does not establish capacity achievability under BP decoding, it provides a theoretical foundation for investigating practical iterative decoding algorithms for the proposed construction.


The remainder of the paper is organized as follows. 
Section~\ref{sec:Preliminaries} introduces the necessary background on CSS codes, Pauli channels, and the classical code ensembles considered in this work.
Section~\ref{sec:main_results} presents 
Section~\ref{sec:constructionA} introduces Construction~A and investigates its ML decoding performance numerically.
Section~\ref{sec:constructionB} develops Construction~B and provides the analytical weight-distribution and capacity-achievability results.
Finally, Section~\ref{sec:conclusion} summarizes the main findings and discusses possible directions for future work. Additional technical results and proofs are provided in the appendices.




